Decidability of Equivalence of Aggregate Count-Distinct Queries

We address the problem of equivalence of count-distinct aggregate queries, prove that the problem is decidable, and can be decided in the third level of Polynomial hierarchy. We introduce the notion of core for conjunctive queries with comparisons as an extension of the classical notion for relational queries, and prove that the existence of isomorphism among cores of queries is a sufficient and necessary condition for equivalence of conjunctive queries with comparisons similar to the classical relational setting. However, it is not a necessary condition for equivalence of count-distinct queries. We introduce a relaxation of this condition based on a new notion, which is a potentially new query equivalent to the initial query, introduced to capture the behavior of count-distinct operator.

==> general-aggregate-queries-k.tex <==


\section{General Aggregate Queries over $K-$Relations}




Consider a conjunctive query with comparisons
$q(\bar{x})\deq A(\bar{x}, \bar{y})$. The answer of $q$ over a given
K-database $D$ is defined as follows:

%%
\[
\ansk{K}{q, D}(t) = 
\left\{
\begin{array}{ll}
\prod\limits_{R(\bar{y})\in A} \lambda R(\bar{y}) 
&
\text{for }~
\begin{array}{|l}
    D\models\lambda A(\bar{x}, \bar{y}),\\
   t= \lambda \bar{x}\\
\end{array}\\
0 & otherwise;
\end{array}
\right. 
\]
%%

In order to define the semantics of GA-queries, we first give
following definition:
%%
\[
\gatk{\bar{x}, \bar{a}}{K}{q, D} = \{\tup{\bar{b}, k} ~|~ \ansk{K}{q,D}(\bar{a}\bar{b})=k \}
\]
%%
Given a general aggregate query $q(\bar{x},\alpha(\bar{y}))\deq
A(\bar{x},\bar{y},\bar{z})$, we can define its semantics over the
K-database $D$ as follows:

\[
%\gaq{U',U''}{R}(t) = 
\ansk{K}{q,D}(t)=
%%
\left\{
\begin{array}{ll} 
    \Sigma_K ~R(\bar{a}\bar{b}) & 
\text{for }~
    \begin{array}{|l}
      \bar{a}\bar{b} \in \ans{\hat{q}, D},\\
      t = \bar{a}.\gatk{\bar{x}, \bar{a}}{K}{\hat{q}, D}; \\
      \bar{a} \in \ans{\exists \bar{y}. \hat{q}, D}
      \end{array}
    \\
    0 & \text{otherwise;}
\end{array}
\right.
\]



\begin{lemma} 
\label{lem:ga-eqk}
For a given semiring $K$, GA-queries $q(\bar{x},\alpha(\bar{y}))\deq
A(\bar{x},\bar{y},\bar{z})$, and its core
$\hat{q}(\bar{x},\bar{y})\deq A(\bar{x},\bar{y},\bar{z})$, such that
$0<|\bar{x}|$ and $0<|\bar{y}|$, and for all $K$-database instances
$D$ followings hold:

\begin{enumerate}
% \item For all $(\bar{t}, n) \in \hat{q}^D$, there exists
%   $\bar{r}.D_{\bar{r}}\in q^D$ such that there exists $(\bar{s}, n)
%   \in D_{\bar{r}}$, such that $\bar{t}=\bar{r}\bar{s}$;
%%
\item For all $t$, $k>0_K$ such that $\ansk{K}{\hat{q}, D}(t)=k$, there
  exists $\bar{r}$, $\bar{s}$, $k'>0_K$ and $t'$, such that
  $\ansk{K}{q, D}(\bar{t'}) = k'$, and $\bar{t}=\bar{r}\bar{s}$,
  $t'=\bar{r}. \gatk{\bar{x}, \bar{r}}{K}{\hat{q}, D}$, and
  $\tup{\bar{s},k}\in \gatk{\bar{x}, \bar{r}}{K}{\hat{q}, D}$.
%%%%
\item For all $t$, $\bar{s}$, $\bar{s}$, $k>0_k$, $k'>0_k$, such that
  $\ansk{K}{q,D}(t)=k$, $t=\bar{r}.D_r$, and $\tup{\bar{s}, k'}\in
  D_r$, it holds that $\ansk{K}{\hat{q}, D}(\bar{r}\bar{s})=k'$.

\end{enumerate}
\end{lemma}
\begin{proof} 
(1). Lets assume $\ansk{K}{\hat{q}, D}(t)=k$. As a result there exists
exactly one assignment $\lambda$ such that: \\
 $$\prod\limits_{R(\bar{z})\in A} \lambda R(\bar{z})=k,
%%
 D\models\lambda A(\bar{x}, \bar{y}), \text{ and }
%%
 t= \lambda \bar{x}.$$

 Lets define $\bar{r}=\lambda\bar{x}$, and
 $\bar{s}=\lambda\bar{s}$. By definition we know that
 $\bar{r}\in\ans{\exists y. \hat{q}, D}$. From the definition we know
 that $\tup{\bar{s},k}\in\gatk{\bar{x}, \bar{r}}{K}{\hat{q},
   D}$. Consequently, $\ansk{K}{q, D}(\bar{t'}) = k'$ for some $k'\ge k>0_K$.

(2) Lets assume $\ansk{K}{q,D}(t)=k$, for $t=\bar{r}.D_r$, and
$\tup{\bar{s}, k'}\in D_r$. Using the definitions we have
$\tup{\bar{r}\bar{s}, k'} \in \ansk{K}{\hat{q},D}$. Consequently,
$\ansk{K}{\hat{q}, D}(\bar{r}\bar{s})=k'$.
\end{proof}

\begin{theorem} Consider GA-queries $q_1(\bar{x},\alpha(\bar{y}))\deq
  A_1(\bar{x},\bar{y},\bar{z_1})$ and
  \\$q_2(\bar{x},\alpha(\bar{y}))\deq
  A_2(\bar{x},\bar{y},\bar{z_2})$. For all $K$-database instances $D$,
  $\ansk{K}{q_1, D}=\ansk{K}{q_2, D}$, iff $\ansk{K}{\hat{q_1},
    D}=\ansk{K}{\hat{q_2}, D}$.
\end{theorem}
\begin{proof}

  (forth) This direction by definition holds since, the semantics of
  general aggregate queries is defined only based on the the cores of
  the queries.

  (back) Lets assume $\ansk{K}{\hat{q_1}, D}(\bar{t})=k$. From the
  first part of Lemma \ref{lem:ga-eqk} we know that there exists
  $\bar{r}$, $\bar{s}$, $k'>0_K$ and $t'$, such that $\ansk{K}{q_1,
    D}(\bar{t'}) = k'$, and $\bar{t}=\bar{r}\bar{s}$,
  $t'=\bar{r}. \gatk{\bar{x}, \bar{r}}{K}{\hat{q_1}, D}$, and
  $\tup{\bar{s},k}\in \gatk{\bar{x}, \bar{r}}{K}{\hat{q_1}, D}$.  By
  assumption of the Lemma we know that $\ansk{K}{q_2, D}(\bar{t'}) =
  k'$. From the second part of Lemma \ref{lem:ga-eqk} we have
  $\ansk{K}{\hat{q_2}, D}(\bar{t})=k$, which completes the proof.


\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> general-aggregate-queries.tex <==


\section{General Aggregate Queries}
Consider a conjunctive query with comparisons
$q(\bar{x})\deq A(\bar{x}, \bar{y})$. The answer of $q$ over a given
database $D$ is defined as follows:

The answer of $q$ over $D$ in set semantics is defined as follows:
%%
\[
\ans{q, D} = \{\lambda{\bar{x}}~|~D\entails \lambda{A(\bar{x}, \bar{y})} \}
\]
%%
We denote with $\ansa{\bar{d}}{\bar{x}}{q, D}$ the set of assignments
from the free variables of $q$ to active domain of $D$ such that
$D\entails A(\bar{x}, \bar{y})$, and $\lambda(\bar{x})=\bar{d}$:



\[
\ansa{\bar{d}}{\bar{x}}{q, D} = \{~\lambda ~|~ D\entails A(\bar{x},
\bar{y}) \text{ and } \lambda(\bar{x})=\bar{d}~\}.
\]
%%
Now we can define the answer of query $q$ over the database $D$ with
set-bag semantics as follows:
\[
q^D= \{~ (\bar{d}, |\ansa{\bar{d}}{\bar{x}}{q, D}|)~ | ~ \bar{d} \in
\ans{q, D}   \}
\]
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
Syntax of {\it GA-query}:
\[
q(\bar{x},\alpha(\bar{y}))\deq A(\bar{x},\bar{y},\bar{z})
\]
%%
In order to define the semantics of GA-queries, we first give
following definition:
%%
\[
\gat{\bar{a}}{\bar{x}}{q, D} = \{~(\bar{b}, |\ansa{\bar{a}\bar{b}}{\bar{x}\bar{y}}{q, D}|) \} 
\]
%%
Now we can define the semantics of GA-queries as the following nested relation:
\[
q^D = \{ \bar{a}.\gat{\bar{a}}{\bar{x}}{\hat{q}, D} ~|~
\bar{a}\in\ans{\exists{\bar{y}}~\hat{q}, D}\}
\]


\begin{lemma} 
\label{lem:ga-eq}
For a given GA-queries $q(\bar{x},\alpha(\bar{y}))\deq
A(\bar{x},\bar{y},\bar{z})$, and its core
$\hat{q}(\bar{x},\bar{y})\deq A(\bar{x},\bar{y},\bar{z})$, such that
$0<|\bar{x}|$ and $0<|\bar{y}|$ following holds:

\begin{enumerate}
\item For all $(\bar{t}, n) \in \hat{q}^D$, there exists
  $\bar{r}.D_{\bar{r}}\in q^D$ such that there exists $(\bar{s}, n)
  \in D_{\bar{r}}$, such that $\bar{t}=\bar{r}\bar{s}$;
\item For all $\bar{r}.D_{\bar{r}}\in q^D$, for all $(\bar{s}, n) \in
  D_{\bar{r}}$, $(\bar{r}\bar{s}, n) \in \hat{q}^D$.
\end{enumerate}
\end{lemma}
\begin{proof} (1). Lets assume $(\bar{t}, m) \in \hat{q}^D$. By
  definition, $|\ansa{\bar{t}}{\bar{x}\bar{y}}{q, D}|=m$, and $0<m$,
  and $1<|\bar{t}|=|\bar{x}\bar{y}|$. There exist $\bar{r}$ and
  $\bar{s}$ such that $\bar{t}=\bar{r}\bar{s}$, and
  $|\bar{r}|=|\bar{x}|$.  By replacing $\bar{t}$ with
  $\bar{r}\bar{s}$, we have
  (i)~$|\ansa{\bar{r}\bar{s}}{\bar{x}\bar{y}}{q, D}|=m$.
%%
  Moreover, (ii)~ $\bar{r}\in\ans{\exists\bar{y}~q, D}$; otherwise,
  $m$ is needed to be zero.
%%
  Using (i) and (ii), and the semantics of GA-queries, we have there
  exists $\bar{r}.D_{\bar{r}}\in q^D$ such that there exists
  $(\bar{s}, m) \in D_{\bar{r}}$, such that $\bar{t}=\bar{r}\bar{s}$;


  (2) Lets assume $\bar{r}.D_{\bar{r}}\in q^D$, and $(\bar{s}, m) \in
  D_{\bar{r}}$. From the semantics of GA-queries we have
  $|\ansa{\bar{r}\bar{s}}{\bar{x}\bar{y}}{q, D}|=m$. Consequently,
  $(\bar{r}\bar{s},m)\in \hat{q}^D$.
\end{proof}

\begin{theorem} Consider GA-queries $q_1(\bar{x},\alpha(\bar{y}))\deq
  A_1(\bar{x},\bar{y},\bar{z_1})$ and \\$q_2(\bar{x},\alpha(\bar{y}))\deq
  A_2(\bar{x},\bar{y},\bar{z_2})$. $q_1$ and $q_2$ are equivalent iff
  their cores are equivalent.
\end{theorem}
\begin{proof}
  (forth) This direction by definition holds since, the semantics of
  general aggregate queries is defined only based on the the cores of
  the queries.
% Lets assume that $\hat{q_1}$ and $\hat{q_2}$ are
%   equivalent. Lets consider $\bar{r}.D_{\bar{r}}\in q_1^D$, such that
%   $(\bar{s}, n) \in D_{\bar{r}}$. From the second result of Lemma
%   \ref{lem:ga-eq}, we have $(\bar{r}\bar{s}, n) \in
%   \hat{q_1}^D=\hat{q_2}^D$. Using the first result of Lemma
%   \ref{lem:ga-eq}, we have there exists $D' $ such that $\bar{r}.D'\in
%   q_2^D$, such that $(\bar{s}, n) \in D'$. In a similar way we can
%   prove that for all $\bar{r}.D_{\bar{r}}\in q_2^D$, for all
%   $(\bar{s}, n) \in D_{\bar{r}}$ there exists $D'$ such that
%   $\bar{r}.D'\in q_1^D$, and $(\bar{s}, n) \in D'$. Consequently, for
%   all $\bar{r}.D_{\bar{r}}\in q_1^D$ there is extactly one
%   $\bar{r}.D_{\bar{r}}\in q_2^D$, and wise versa. This implies
%   $q_1^D=q_2^D$;

  (back) Lets assume that $q_1(D)$ and $q_2(D)$ are
  equivalent.

  We need to prove that for all $\hat{q_1}(D)$ and $\hat{q_2}(D)$ are
  also equivalent.

Immediate consequnce of the second result of Lemma
  \ref{lem:ga-eq}.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

